Understanding the LLM-ification of CHI: Unpacking the Impact of LLMs at CHI through a Systematic Literature Review

Large language models (LLMs) have been positioned to revolutionize HCI, by reshaping not only the interfaces, design patterns, and sociotechnical systems that we study, but also the research practices we use. To-date, however, there has been little understanding of LLMs' uptake in HCI. We address this gap via a systematic literature review of 153 CHI papers from 2020-24 that engage with LLMs. We taxonomize: (1) domains where LLMs are applied; (2) roles of LLMs in HCI projects; (3) contribution types; and (4) acknowledged limitations and risks. We find LLM work in 10 diverse domains, primarily via empirical and artifact contributions. Authors use LLMs in five distinct roles, including as research tools or simulated users. Still, authors often raise validity and reproducibility concerns, and overwhelmingly study closed models. We outline opportunities to improve HCI research with and on LLMs, and provide guiding questions for researchers to consider the validity and appropriateness of LLM-related work.

==> files/codebook.tex <==



\begin{table}[H]
\centering
\caption{The final codebook with four code categories as well as the Inter-Rater Reliability. Multiple codes can apply to one paper.}
\begin{tabular}{p{4cm}p{9cm}p{2cm}}
\toprule \midrule
\textbf{Category} & \textbf{Codes} & \textbf{IRR} \\
\midrule 
Contribution Types (7 codes) & Empirical, Artifact, Methodological, Theoretical, Dataset, Metareview, Opinion & \textbf{0.866} \\ \midrule
Application Domain (10 codes) & Communication \& Writing, Augmenting Capabilities, Education, Responsible Computing, Programming, Reliability \& Validity of
LLMs, Well-being \& Health,  Design, Accessibility \& Aging, Creativity & \textbf{0.849} \\ \midrule
Roles of LLMs (5 codes) & LLMs as system engines; LLMs as research tools; LLMs as participants \& users; LLMs as objects of study; Users' perceptions of LLMs  & \textbf{0.773} \\ \midrule
Limitations \& Risks (29 codes) & \textbf{Limitations on LLM Performance} LLM bias toward different groups, limited data coverage in the training data, non-deterministic response, hallucination, unspecificied errors and biases; \textbf{Limitations on Research Validity} internal and/or external validity across users, contexts, models, prompts; \textbf{Limitations on Resource} computational cost, financial cost, lack of evaluation standards; \textbf{Risks to Society, consequences} economic harms, representational harms, misinformation harms, malicious use, hate speech, and environmental harms. &
\textbf{0.887} (\textbf{0.633} for the 29 low-level codes)  \\ 

& \textbf{Note}: \textit{There are 22 low-level codes described in the full paper. However, we had an initial set of 29 low-level code. We had four code ``others'' under each coarse categories (e.g., other LLM performance issues). We also merged three other codes during the coding process (i.e., latency, lack of access to open/close models, prompt-induced performance issues). These codes overlap with the definition of the 22 main codes.}
\\
\midrule

% Non-determinstric reponse; Hallucination; LLM bias toward different groups; Unspecified errors; limits of LLM data coverage; latency; other technical bugs; Internal/External Validity across Users/Contexts/Models/Prompts; Financial Cost; Computational Cost; Open v. Closed models; Proposed modularity without evaluation; Lack of evaluation standards/metrics; Environmental cost; representational harms; privacy; misinformation; malicious use; hate speech & \textbf{0.633}\footnote{\textbf{0.887} for the four coarse-level codes}  \\ \midrule
\bottomrule
\end{tabular}
\end{table}

% Roles of LLMs (5 codes) & (1) LLMs powers the system; (2) LLMs infers user intent; (3) LLMs simulates user behaviors; (4) LLMs improve users’ creativity; (5) LLMs change how users interact with LLMs themselves; (5) study how users use and/or perceive LLMs (systems)  & \textbf{0.773} \\ \midrule


==> tables/analysis.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{files/analysis.jpeg}
    \caption{The open coding process to answer our research questions during the meta-review.}
    \label{fig:analysis-process}
\end{figure}

==> tables/frequency.tex <==
\begin{table}[h!]
\centering
\caption{The frequency of applied codes for \emph{application areas}, \emph{contribution types}, and \emph{LLM roles}}
\begin{tabular}{p{3.2cm}l|p{2cm}l|ll}
\toprule
\textbf{Application areas} & Papers & \textbf{Contribution type} & Papers & \textbf{LLM roles} & Papers \\
\midrule
Communication \& Writing & 34 (22.7\%) & Empirical & 148 (98.7\%) & LLMs power the System & \\
Augmenting Capabilities & 26 (17.3\%) & Artifact & 92 (61.3\%) & LLMs as Research Assistants & \\
Education & 22 (14.7\%) & Methodological & 15 (10.0\%) & LLMs as participants/Users & \\
Responsible Computing & 18 (12\%) & Theoretical & 8 (5.3\%) & LLMs themselves being studied & \\
Software Engineering & 17 (11.3\%) & Dataset & 6 (4.0\%) & Users' Perceptions of LLMs & \\
Reliability \& Validity of LLMs & 16 (10.7\%) & & & & \\
Well-being \& Health & 14 (9.3\%) & & & & \\
Design & 13 (8.7\%) & & & & \\
Accessibility & 12 (8.0\%) & & & & \\
Creativity & 9 (6.0\%) & & & & \\
\bottomrule
\end{tabular}
\label{tab:frequency}
\end{table}

